Post-processing output from ensembles with and without parametrised convection, to create accurate, blended, high-fidelity rainfall forecasts

Flash flooding is a significant societal problem, but related precipitation forecasts are often poor. To address this, one can try to use output from convection-parametrising (global) ensembles, post-processed to forecast at point-scale, or convection-resolving limited area ensembles. In this study, we combine both. First, we apply the "ecPoint-rainfall" post-processing to the ECMWF global ensemble. Then, we use 2.2km COSMO LAM ensemble output (centred on Italy), and also post-process it using a scale-selective neighbourhood approach to compensate for insufficient members. The two components then undergo lead-time-weighted blending, to create the final probabilistic 6h rainfall forecasts. Product creation for forecasters constituted the "Italy Flash Flood use case" within the EU-funded MISTRAL project and it will be a real-time open-access product. One year of verification shows that ecPoint is the most skilful ensemble product. The post-processed COSMO ensemble adds most value to summer convective events in the evening, when the global model has an underprediction bias. In two heavy rainfall case studies we observed underestimation of the largest point totals in the raw ECMWF ensemble, and overestimation in the raw COSMO ensemble. However, ecPoint increase the value and highlighted best the most affected areas, whilst post-processing of COSMO diminished extremes by eradicating unreliable detail. The final merged products looked best from a user perspective and seemed to be the most skilful of all. Although our LAM post-processing does not implicitly include bias correction (a topic for further work) our study nonetheless provides a unique blueprint for successfully combining ensemble rainfall forecasts from global and LAM systems around the world. It also has important implications for forecast products as global ensembles move ever closer to having convection-permitting resolution.

==> header.tex <==
% Add any additional LaTeX packages and macros here
\usepackage{siunitx}

%---

\iflatexml
% Add any LateXML specific commands here

%---

\else
% The commands below will only change the exported PDF. Edit or remove as needed

\usepackage{lineno}
\linenumbers

\renewcommand{\sfdefault}{ptm}
\renewcommand{\familydefault}{\sfdefault}


\paperfield{Field of the paper}
\abbrevs{ABC, a black cat; DEF, doesn't ever fret; GHI, goes home immediately.}
\corraddress{Est\'ibaliz Gasc\'on, European Centre for Medium-Range Weather Forecasts, Reading, United Kingdom}
\corremail{estibaliz.gascon@ecmwf.int}
\presentadd{Department, Institution, City, State or Province, Postal Code, Country}
\fundinginfo{This work has been supported by the MISTRAL project under the Connection Europe Facility (CEF) Telecommunication Sector Programme of the European Union}
\fi

%---
